Constraining the observer angle of the kilonova AT2017gfo associated with GW170817: Implications for the Hubble constant

There is a strong degeneracy between the luminosity distance ($D_L$) and the observer viewing angle ($\theta_{\rm obs}$; hereafter viewing angle) of the gravitational wave (GW) source with an electromagnetic counterpart, GW170817. Here, for the first time, we present independent constraints on $\theta_{\rm obs} = 32.5 ^{\circ +11.7}_{-9.7}$ from broad-band photometry of the kilonova (kN) AT2017gfo associated with GW170817. These constraints are consistent with independent results presented in the literature using the associated gamma ray burst GRB170817A. Combining the constraints on $\theta_{\rm obs}$ with the GW data, we find an improvement of 24$\%$ on $H_0$. The observer angle constraints are insensitive to other model parameters, e.g. the ejecta mass, half-opening angle of the lanthanide-rich region and the temperature. A broad wavelength coverage extending to the near infrared is helpful to robustly constrain $\theta_{\rm obs}$. While the improvement on $H_0$ presented here is smaller than the one from high angular resolution imaging of the radio counterpart of GW170817, kN observations are significantly more feasible at the typical distances of such events from current and future LIGO-Virgo Collaboration observing runs ($D_L \sim 100$ Mpc). Our results are insensitive to the assumption on the peculiar velocity of the kN host galaxy.

==> alt_dataset_results.tex <==
\begin{table}
    \caption{The table showing the impact of only using a subset of the data for computing the \costh distribution. 
    UVOIR refers to the entire wavelength range observed, OIR is without the UV and UVO is without the NIR. For the analyses without early time data, the phase ranges are given in parenthesis}

    \centering
    \resizebox{.45\textwidth}{!}{\begin{tabular}{|c|c|c|c|}
    \hline
    Model fit & Data Sample & Median H$_0$ & Improvement\\
        & & (km s$^{-1}$Mpc$^{-1}$) & ($\%$)\\
    \hline
    \hline
    
    
    %UVOIR (t $< 7$\,d) & Best & 75.1 & 18\\
    %--- & \ejm, $\Phi$, T & 74.9 & 11\\
    %--- & \ejm & 75.8 & 11\\
    %--- &  $\Phi$ & 73.9 & 18\\
    %--- &  T & 75.1 & 18\\
    OIR (t $< 7$\,d) & Best & 72.0 & 24\\
    --- & \ejm, $\Phi$, T & 70.7 & 18\\
    UVO (t $< 7$\,d) & Best & 70.6 & 30\\
    --- & \ejm, $\Phi$, T & 70.7 & 18\\ 
    UVOIR ($1\,{\rm d} <$ t $< 7$\,d) & Best & 72.1 & 20\\
    --- & \ejm, $\Phi$, T & 71.7 & 4\\
    UVOIR ($2\,{\rm d} <$ t $< 7$\,d) & Best & 73.6 & 3\\
    --- & \ejm, $\Phi$, T & 71.9 & 0\\
    UVOIR ($3\,{\rm d} <$ t $< 7$\,d) & Best & 71.7 & 3\\
    --- & \ejm, $\Phi$, T & 71.3 & 0\\
    UVOIR (t $< 10$\,d) & Best & 72.4 & 18\\
    --- & \ejm, $\Phi$, T & 71.9 & 11\\
    \hline
    {\bf UVOIR} & {\bf Best} &  {\bf 72.5} & {\bf 22}\\
    \hline
    \end{tabular}}
    \label{tab:results_alt}
\end{table}

==> results_tab_old.tex <==
\begin{table}
    \caption{The table summarises the H$_0$ values for the different \texttt{POSSIS} model parameters marginalised over for calculating the synthetic observables.}

    \centering
    \begin{tabular}{|c|c|}
    \hline
    Model fit & H$_0$\\
        & (km s$^{-1}$Mpc$^{-1}$)\\
    \hline
    \hline
    Best     &  72.5$^{+8.8}_{-8.5}$\\
     \ejm, $\Phi$, T & 70.9$^{+10.5}_{-6.2}$\\
    \ejm &   72.2$^{+10.3}_{-6.3}$\\
    $\Phi$  & 71.1$^{+9.0}_{-6.4}$\\
    T & 72.4$^{+9.1}_{-6.3}$\\
    %Best     &  75.1$^{+7.0}_{-9.1}$\\
    % \ejm, $\Phi$, T & 74.9$^{+7.6}_{-10.2}$\\
    %\ejm &   75.8$^{+7.4}_{-10.2}$\\
    %$\Phi$  & 73.9$^{+7.2}_{-9.1}$\\
    %T & 75.1$^{+7.0}_{-9.1}$\\
    \hline
    {\bf GW only} & {\bf 70.0$^{+12.2}_{-7.8}$} \\
    \hline
    \end{tabular}
    \label{tab:results}
\end{table}
